A New Study of s-Process Nucleosynthesis in Massive Stars

We present a comprehensive study of s-process nucleosynthesis in 15, 20, 25, and 30 $\msun$ stellar models having solar-like initial composition. The stars are evolved up to ignition of central neon with a 659 species network coupled to the stellar models. In this way, the initial composition from one burning phase to another is consistently determined, especially with respect to neutron capture reactions. The aim of our calculations is to gain a full account of the s-process yield from massive stars. In the present work, we focus primarily on the s-process during central helium burning and illuminate some major uncertainties affecting the calculations. We briefly show how advanced burning can significantly affect the products of the core helium burning s-process and, in particular, can greatly deplete $^{80}$Kr that was strongly overproduced in the earlier core helium burning phase; however, we leave a complete analysis of the s-process during the advanced evolutionary phases (especially in shell carbon burning) to a subsequent paper. Our results can help to constrain the yield of the s-process material from massive stars during their pre-supernova evolution.

==> figcaption.tex <==
%auto-ignore
%---------------------------------------------------------------------
\clearpage

\figcaption{
Evolution of the central temperature vs. central density for the four case
A stellar models.
The temperature scale,
$\tilde{T}_C$ is $\approx$ 2$\times$10$^7 \; \rho^{1/3}$.
All four star models have been evolved up to central neon ignition.
\label{fig:TCvsRhoC} }


\figcaption{
The convective helium-burning core mass in the four case A star models versus
the fraction of the helium-burning time (upper panel) and the mass fraction
of $^4$He (lower panel).
Starting at X($^4$He) = 0.1, the edges of the convective cores have been
finely resolved to prevent a sudden injection of a large supply of
$^4$He into the cores.
\label{fig:MconvXHe}
}



\figcaption{
Several s-process diagnostics for two 25 $M_\odot$ stellar models.
The case A model is shown as the solid curve while the case B model
is shown as the dashed line.
The diagnostics are the following: 
a) $\tau_n$ is the central neutron exposure, as computed from Eq.
(\protect\ref{eq:taun}).  It is the neutron exposure that would have been
seen by a nucleus that stayed
in the center of the star throughout the burning ($\tau_n$).
$\tau_{54}$  is the neutron
exposure computed from the decline of the $^{54}$Fe abundance
due to neutron captures (see Eq. [\protect\ref{eq:tau54}]).  
The latter better indicates the average neutron exposure
of the core helium-burning s-process because it reflects the dilution by
the convective
mixing.  It also shows that the bulk of the s-processing occurs mainly in
the range X($^{4}$He)$_C$ $\simeq$ 0.01 - 0.001.
b) Overabundances of key isotopes. Note that the production factor of
$^{22}$Ne is multiplied by 1/100 in order that it not overlap 
in the figure that of $^{25}$Mg.
c) The number of neutrons captured per iron-seed nucleus according to Eq.
(\protect\ref{eq:nc}). 
d) The central neutron density of the star during core helium burning.  
All quantities are plotted against central helium mass fraction.
A low-lying $^{22}$Ne($\alpha$,n)$^{25}$Mg resonance (case B) would 
dramatically increase the robustness of the core helium-burning s-process.
\label{fig:centralsproc25Msun}
}



\figcaption{
The central neutron density as function of central helium mass fraction
or time for the four case A (top panel) and the four case B (lower panel)
stellar models.
\label{fig:centndnsvsXHe}
}



\figcaption{
The neutron exposure $\tau_n$ as a function of interior mass for all
eight case A (solid curve) and B (dashed curve)
stellar models through core helium burning.  
$\tau_n$ is the neutron exposure a nucleus would experience were it
to remain at the particular interior mass.
This figures clearly demonstrates that most neutron captures occur
in the very center of the star.  
Nuclei are convected down into the center of the star, capture neutrons, 
and then mix back out into the core.
\label{fig:tauneutvsMr}
}


\figcaption{
Similar to Figure \protect\ref{fig:centralsproc25Msun} but for
the case A (solid curve), case C (long-dashed curve), and case D (short-dashed
curve) 20 M$_{\sun}$ stellar models.
The lowest $^{12}{\rm C}(\alpha,\gamma)^{16}$O reaction rate gives the
largest degree of s-processing.  The results of cases A and D agree to
within $\sim 10-20\%$.
\label{fig:centralsproc20Msun}
}


\figcaption{
Overabundances of heavy nuclei (mass number $A\geq 12$) averaged over the
convection helium-burning core for the four case A stellar models.
The primary nucleosynthesis production process for each
isotope is indicated by the symbol type.
\label{fig:prodfactRCF88}
}

\figcaption{
Overabundances of heavy nuclei (mass number $A\geq 12$) averaged over the
convection helium-burning core for the 25 $M_\odot$ stellar model with
10\% contribution to the reaction rate for $^{22}{\rm Ne}(\alpha,n)^{25}$Mg
from a low-lying resonance.
\label{fig:prodfact25}
}


\figcaption{
Several s-process diagnostics for the 25 $M_\odot$ case A stellar model
at central neon ignition.  
The upper panel shows the two measures of the neutron exposure.
Of particular interest is the run of $\tau_n$ against interior mass.
The dashed line shows the conditions at the end of core helium burning,
while the solid line shows the conditions at the end of core neon burning.
Most s-processing has occurred in the center of the star, but the contribution
from shell carbon burning and shell helium burning are evident at 1.6
$M_\odot$ and about 5.4 $M_\odot$, respectively.  
The middle panel shows the
number of neutrons captured per iron seed nucleus and the overabundance of
$^{80}$Kr at the end of core helium (dashed line) and neon burning (solid
line).  
Various convective burning phases after central helium burning
modify the number of neutrons captured per seed nucleus.
Interestingly, shell carbon s-processing has destroyed a significant
fraction of the $^{80}$Kr produced in earlier convection core helium
burning.
The bottom panel shows mass fractions at the end of core neon burning
of some nuclei to indicate the nuclear burning region.
\label{fig:kr80Cshell}
}



%---------------------------------------------------------------------
\clearpage


